SPARK-IL: Spectral Retrieval-Augmented RAG for Knowledge-driven Deepfake Detection via Incremental Learning

Detecting AI-generated images remains a significant challenge because detectors trained on specific generators often fail to generalize to unseen models; however, while pixel-level artifacts vary across models, frequency-domain signatures exhibit greater consistency, providing a promising foundation for cross-generator detection. To address this, we propose SPARK-IL, a retrieval-augmented framework that combines dual-path spectral analysis with incremental learning by utilizing a partially frozen ViT-L/14 encoder for semantic representations alongside a parallel path for raw RGB pixel embeddings. Both paths undergo multi-band Fourier decomposition into four frequency bands, which are individually processed by Kolmogorov-Arnold Networks (KAN) with mixture-of-experts for band-specific transformations before the resulting spectral embeddings are fused via cross-attention with residual connections. During inference, this fused embedding retrieves the $k$ nearest labeled signatures from a Milvus database using cosine similarity to facilitate predictions via majority voting, while an incremental learning strategy expands the database and employs elastic weight consolidation to preserve previously learned transformations. Evaluated on the UniversalFakeDetect benchmark across 19 generative models -- including GANs, face-swapping, and diffusion methods -- SPARK-IL achieves a 94.6\% mean accuracy, with the code to be publicly released at https://github.com/HessenUPHF/SPARK-IL.

==> acronyms.tex <==
\section*{Acronyms}
\begin{acronym}[UFD]
  \acro{FFT}{Fast Fourier Transform}
  \acro{KAN}{Kolmogorov--Arnold Network}
  \acro{RAG}{Retrieval--Augmented Generation}
  \acro{ViT}{Vision Transformer}
  \acro{EWC}{Elastic Weight Consolidation}
  \acro{ACC}{Accuracy}
  \acro{mAcc}{Mean Accuracy}
  \acro{GFLOPs}{Giga Floating--Point Operations}
  \acro{CLIP}{Contrastive Language--Image Pretraining}
  \acro{tSNE}{t--distributed Stochastic Neighbor Embedding}
  \acro{GAN}{Generative Adversarial Network}
  \acro{LDM}{Latent Diffusion Model}
\end{acronym}

